DarkFlux: A new tool to analyze indirect-detection spectra of next-generation dark matter models

We present DarkFlux, a software tool designed to analyze indirect-detection signatures for next-generation models of dark matter (DM) with multiple annihilation channels. Version 1.0 of this tool accepts user-generated models with $2\to 2$ tree-level dark matter annihilation to pairs of Standard Model (SM) particles and analyzes DM annihilation to $\gamma$ rays. The tool consists of three modules -- the annihilation fraction module, the flux module, and the analysis module -- which can be run in a loop in order to scan over DM mass if desired. [A description of each module is available in the full abstract.] DarkFlux v1.0 compares the total $\gamma$-ray flux to a joint-likelihood analysis of fifteen dwarf spheroidal galaxies (dSphs) analyzed by the $Fermi$-LAT collaboration. DarkFlux automatically provides data tables and can plot the output of the three modules. In this manual, we briefly motivate this indirect-detection computer tool and review the essential DM physics. We then describe the several modules of DarkFlux in greater detail. Finally, we show how to install and run DarkFlux and provide two worked examples demonstrating its capabilities.

==> TeX/running.tex <==
\section{Running DarkFlux}\label{srun}

\subsection{inputs}

We now briefly describe the input and output files as \textsc{DarkFlux} is run.  The input requires a user generated model file in UFO format which the user must place in the Madgraph models folder. The user must now specify the inputs to \textsc{DarkFlux}  found in the file \textsf{run\textunderscore input.dat}. There are 6 field options to be specified in the  \textsf{run\textunderscore input.dat}  file. 
\\
\begin{itemize}

\item {As \textsc{DarkFlux} automatically scans over dark matter masses, the first entry field option sets the scan parameters for dark matter masses, number of steps and step size. The parameter  \textsf{Mdm\textunderscore i} sets the initial dark matter mass. The parameter \textsf{limit} specifies the number of dark matter mass steps to be made, and the parameter \textsf{step} specifies the step size in GeV.  }


\item{Next the user must specify the pointer to the user generated model. Thus the user must set the parameter \textsf{model\textunderscore name} to the appropriate corresponding Madgraph model name which is that same as the one that appears in the Madgraph models folder.}


\item{The next two fields set the dark matter particle name (\textsf{dm\textunderscore name}) and the dark matter mass tag (\textsf{dm\textunderscore mass\textunderscore name}) to the appropriate values specified in the \textsf{particles.dat} and \textsf{parameters.dat} files of the user generated  Madgraph model UFO.}


\item{The next field chooses the appropriate MadDM mode in which to compute the velocity averaged cross sections. Since MadDM is only used for cross section computation fast mode is recommended.}


\item{The final input field allows the user to set various parameter values in the UFO model file. These may correspond, for example, to various mediator masses or couplings.  The user may set any number of model parameters in this way.  The user specifies the name of the parameters \textsf{parameter\textunderscore tagi} which corresponds to the name of the same parameters in the \textsf{parameters.dat} file of the user generated UFO in the Madgraph models folder.}

\end{itemize}

\subsection{outputs}
\textsc{DarkFlux} outputs 5 files which reside in the folder \textsf{idtool/spectrabymass/results}. These files are  \textsf{results.txt}, \textsf{xsec\textunderscore limits.dat}, \textsf{ratebymass.pdf}, \textsf{spectrumbymass.pdf}, and  \textsf{ratebymass.pdf}.
\\

We will first describe the output file \textsf{results.txt}, a simple text file is generated which contains 4 fields. 

\\
\begin{itemize}
\item The first field is simply the dark matter mass. 

\item The second field is a list of partial annihilate rates in 16 channels. The rates in the channels are as specified 

\item The next field is the value \textsf{sv} which is the 95 percent confidence upper limit of velocity averaged cross section by the Fermi dwarf galaxy analysis for the dark matter mass in question.  

\item Finally the energy spectrum is given specifying the total photon yield in each of twenty four energy bins.


\end{itemize}
 


The file \textsf{xsec\textunderscore limits.dat} contains a table which lists the computed upper limit on the velocity averaged cross section for each scanned dark matter mass.
\\

The final three files are visualization plots created by python. First the plot, \textsf{ratebymass.pdf}, plots the partial annihilation rates $R_i$ vs. scanned dark matter mass for each channel.  Next, the program generates file \textsf{spectrumbymass.pdf} which plots the total photon flux spectrum for each dark matter mass. Finally \textsc{DarkFlux} generates the plot \textsf{ratebymass.pdf} which plots the computed 95 percent upper limit on the thermally averaged annihilation cross section vs dark matter mass.  

